Towards Open-World Recommendation with Knowledge Augmentation from Large Language Models

Recommender systems play a vital role in various online services. However, the insulated nature of training and deploying separately within a specific domain limits their access to open-world knowledge. Recently, the emergence of large language models (LLMs) has shown promise in bridging this gap by encoding extensive world knowledge and demonstrating reasoning capability. Nevertheless, previous attempts to directly use LLMs as recommenders have not achieved satisfactory results. In this work, we propose an Open-World Knowledge Augmented Recommendation Framework with Large Language Models, dubbed KAR, to acquire two types of external knowledge from LLMs -- the reasoning knowledge on user preferences and the factual knowledge on items. We introduce factorization prompting to elicit accurate reasoning on user preferences. The generated reasoning and factual knowledge are effectively transformed and condensed into augmented vectors by a hybrid-expert adaptor in order to be compatible with the recommendation task. The obtained vectors can then be directly used to enhance the performance of any recommendation model. We also ensure efficient inference by preprocessing and prestoring the knowledge from the LLM. Extensive experiments show that KAR significantly outperforms the state-of-the-art baselines and is compatible with a wide range of recommendation algorithms. We deploy KAR to Huawei's news and music recommendation platforms and gain a 7\% and 1.7\% improvement in the online A/B test, respectively.

==> backup.tex <==
\section{Preliminaries}
In this section, we formulate the general recommendation task and describe 
Click-through rate (CTR) prediction is a crucial task in recommender systems, sharing similar input-output characteristics with many recommendation tasks. In this work, we focus on CTR prediction as the basic task of our framework and this section introduce its formulation and the basic structure. However, it is important to note that our framework is extendable to other recommendation tasks as well.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{imgs/promptV3.pdf}
    \caption{Prompts designed under our framework (some text has been omitted due to the page limits).}
    \label{fig:promp}
\end{figure*}

\subsection{Task Formulation} 
CTR prediction can be formulated mathematically as a binary classification problem over multi-field categorical feature data. The dataset is denote as $D = \{(x_1, y_1), \ldots, (x_i, y_i), \ldots, (x_n, y_n)\}$, where $x_i$ represents the categorical features for the $i$-th instance and $y_i$ denotes the corresponding binary label (0 for no-click and 1 for click). Usually, $x_i$ contains sparse one-hot vectors from multiple fields, such as item id and genre. We can represent the feature as $x_i=[x_{i,1}, x_{i,2},\ldots,x_{i, F}]$ with $F$ being the number of field and $x_{i, f}$, $f=1,\ldots,F$ being the feature of corresponding field. 

The goal of CTR prediction is to learn a function that can accurately predict the click probability $P(y_i=1|x_i)$ for each sample. The traditional framework focusing on feature interaction \cite{DCN,DeepFM,FiBiNET, AutoInt} is formulated as
\begin{equation}
    \hat{y_i} = f(x_i;\theta)\,,
     \label{eq:ctr-goal-1}
\end{equation}
where $f$ is the learned function with parameters $\theta$. However, there are also CTR prediction \cite{DIN, DIEN} models that emphasize sequential behavior modeling and incorporate the user behavior sequence $h_i$ prior to the current prediction sample $x_i$, so the framework can also be formulated as
\begin{equation}
    \hat{y_i} = f(x_i,h_i;\theta)\,.
     \label{eq:ctr-goal-2}
\end{equation}

\subsection{Basic Structure of CTR Model}
According to \cite{zhang2021deep}, most recent CTR models may typically have the following four layers: (1) embedding layer, (2) feature interaction layer, (3) user behavior modeling layer, and (4) output layer. The \textbf{embedding layer} coverts categorical features into low-dimensional dense embeddings, that is to transform $x_{i,j}$ into $e_{i,j}$ so as to get the embedding $e_i=[e_{i,1};e_{i,2};\ldots;e_{i,F}]\in\mathbb{R}^{F\times d}$ of $i$-th instance with $d$ being the embedding size. The \textbf{feature interaction layer} combines embeddings and other continuous features to capture complex relationships and high-order interactions, enabling the model to learn non-linear patterns. The \textbf{user behavior modeling layer} models user interests and preferences based on historical behavior or contextual information, utilizing techniques like RNNs or attention mechanisms to capture temporal dynamics and long-term dependencies. The \textbf{output layer} takes the processed features and generates the final prediction or click probability, usually using a linear or MLP layer followed by a sigmoid activation function.


Note that not all models include all four components mentioned above. Depending on whether the model emphasizes sequence modeling or feature interactions, it may have either the feature interaction layer or the interest modeling layer. After obtaining the predictions from the output layer, the model is typically trained with Binary Cross-Entropy (BCE) loss:
\begin{equation}
\mathcal{L}=\sum_{i=1}^n y_{i}\log \hat{y}_{i} + (1-y_{i})\log(1-\hat{y}_{i})\,.
\end{equation}

% \textbf{Embedding layer} is responsible for transforming categorical features into low-dimensional dense embeddings, that is to transform $x_{i,j}$ into $e_{i,j}$ so as to get the embedding $e_i=[e_{i,1};e_{i,2};\ldots;e_{i,F}]\in\mathbb{R}^{F\times d}$ of $i$-th instance with $d$ being the embedding size.


% \textbf{Feature interaction layer} combines the embeddings and possibly other continuous features to capture complex relationships and high-order interactions between different features. It applies operations like inner/outer product, neural network, and attention, allowing the model to capture non-linear patterns and interactions within the data.

% \textbf{User behavior modeling layer} focuses on modeling the user's interests and preferences based on historical behavior or contextual information. It can incorporate techniques like recurrent neural networks (RNNs) or attention mechanisms to capture temporal dynamics and long-term dependencies in the user's sequential behavior, providing a accurate representation of user interests.


% \textbf{Output layer} takes the processed features from the previous layers and produces the final prediction or click probability. It typically involves a single linear or MLP layer followed by a sigmoid activation function, representing the estimated probability of a user clicking on a specific item or advertisement. 




\section{Methodology}
We first introduce the overview of our proposed model-agnostic framework, followed by the elaborate detail of each component.
% Model-Agnostic LLM-enhanced
\subsection{Overview}
To extract open-world knowledge from LLM and incorporate it into traditional recommendation systems, we design OpenRec, as shown in Figure~\ref{fig:open_world}. This framework is model-agnostic and consists of the following stages: \textbf{1) Knowledge Reasoning and Generation Stage} leverages prompt to extract recommendation-relevant knowledge from LLM. We first decompose user interests into different factors and allow LLM to do preference reasoning based on these factors and user's historical behaviors. Simultaneously, LLM will generate aligned knowledge of candidate items based on relevant factors.  \textbf{2) Knowledge Adaptation Stage} involves converting textual knowledge into more compact and relevant representations suitable for recommendation, bridging the gap between LLM and RS. First, the textual knowledge obtained above is encoded into dense representations by text encoder. Next, a semantic transformation module is adopted to transform the representations from the semantic space to the recommendation space to obtain user preference representations and item knowledge representations of candidate items. \textbf{3) Knowledge Utilization Stage} integrates the extracted user preference and item knowledge representation into the existing recommendation model, enabling it to leverage both domain knowledge and open-world knowledge during the recommendation process. 

 Overall, this framework aims to leverage the open-world knowledge and reasoning ability of LLM and incorporate it to traditional recommendation models efficiently. The knowledge reasoning and generation stage, as well as the encoding of generated knowledge, can be preprocessed and stored for efficient retrieval. The semantic transformation module will be jointly trained with the backbone recommendation model to ensure efficient inference. 
% \subsection{Knowledge and Preference Extraction }
\subsection{Knowledge Reasoning and Generation}

% LLM-augmented Representation
Reasoning is a fundamental part of human intelligence that provide back-end support for various real-world applications. In the field of recommendation, the ability to reason is also crucial since it allows us to go beyond the simple correlations and uncover underlying patterns and connections in user behaviors. It helps us understand the "why" behind user preferences and enables more accurate and personalized recommendations. However, traditional recommendation models primarily focus on leveraging statistical techniques and collaborative signals because modern neural networks can hardly reason from the input data. Fortunately, with the revolutionary development of pre-training and the scaling up of model size, LLMs has shown emergent behaviors such as the reasoning ability~\cite{qiao2023reasoning,huang2022reasoning}. This opens up new possibilities for incorporating reasoning in recommendation system.
\subsubsection{Scenario-specific Preference Decomposition} While LLMs excel at capturing underlying correlations and patterns, they may struggle to directly handle complex reasoning tasks consisting of multiple problems. According to~\cite{press2022measuring}, LLMs often suffers from \textit{compositional gap} that the model do not generate the correct answer to the compositional question but can correctly answer all its sub-questions. Unfortunately, inferring user's preferences belongs to such compositional problem involving multiple reasoning steps and composing multiple facets of user interest. Thus, LLMs may not be bale to directly do preference reasoning accurately and previous work~\cite{liu2023chatgpt,chatrec,hou2023large} that expects LLMs to directly provide precise answer to the user preference might be overly ambitious. 

Motivated by~\cite{press2022measuring, zhou2023leasttomost} that decompose complex problem in sub-problems, we propose to decompose user preference into different factors and employ LLM to predict according to those factors. Specifically, different scenarios or recommendation domains may require the consideration of distinct factors, prompting us to employ different preference decomposition approaches for different scenarios. For instance, in movie recommendation, we take into account factors like genre, actors, directors, theme, mood, production quality, and critical acclaim. Similarly, in new recommendation, we consider topic, source, region, style, freshness, etc. To determine the specific factors for different scenarios, we rely on a combination of expert opinions and interactive collaboration with LLM. This collaborative process between experts and LLM ensures that the chosen factors encompass the critical dimensions of user preference for each scenario.

By breaking down user preference, we help LLMs recall more detailed knowledge and make the preference reasoning task more manageable for LLM, therefore addressing the limitations of direct preference reasoning of LLM.


% Such complex reasoning ability is usually unlocked by specific prompting strategies, e.g., generated knowledge prompting~\cite{}, and problem decomposition ~\cite{}. 
\subsubsection{LLM as Preference Reasoner \& Knowledge Provider}
After obtaining the scenario-specific preference factors, we incorporate them in to the design of prompts in utilizing LLM as a preference reasoner and knowledge provider. As illustrated in Figure~\ref{fig:promp}, we design two types of prompts: preference prompt and item prompt, which facilitate the preference reasoning process of LLM and the extraction of preference-related knowledge of items from LLM.

\textbf{Preference prompt} is constructed with user's description, historical behaviors, and scenario-specific preference factors. Next, LLM takes in the prompt and generate \textbf{preference knowledge} related to preference factors.  As shown in Figure~\ref{fig:promp}, the user description, historical behaviors provide LLM with the necessary context and user-specific information to understand the user's preference. The scenario-specific  factors reduce the difficulty of reasoning and allows the LLM to recall the relevant knowledge better and more comprehensively. Hence we can observe that in the generated preference knowledge, LLM gives the user's preferences for the corresponding factor based on the user's behavior.

\textbf{Item prompt} are designed to fill in the missing knowledge gap between candidate item and generated preference knowledge. Since the dataset of recommender system may lack relevant knowledge about preference factors from items, we need to extract corresponding knowledge from LLM for alignment. As illustrated in Figure~\ref{fig:promp}, the item prompt consists of two parts the given item description and scenario-specific preference factors. By constructing item prompt in this manner, LLM can generate \textbf{item knowledge} that aligns with preference factors, allowing for more accurate and contextually recommendation.

By combining of the two kinds of prompts, we create a framework where LLM acts as both preference reasoner and knowledge provider, successfully extracting open-world knowledge from LLM that benefits for recommender system.
\subsection{Knowledge Adaptation}
The knowledge generated by LLM presents new challenges in harnessing its potential to assist in recommendations. Several key factors complicate the utilization of this knowledge: 1) The knowledge generated by LLM usually exists in the form of text, which cannot be directly leveraged by traditional RS that typically processes categorical features. 2) Even if some LLMs are open-sourced, the decoded outputs are usually large dense vectors (e.g., 4096 for each token) and belong to a semantic space that differs significantly from the recommendation space. This mismatch poses a significant challenge in directly utilizing them in RS. 3) Furthermore, the generated knowledge may contain noise or unreliable information~\cite{ji2023survey}. 

To address these challenges, we have devised two modules: \textbf{knowledge encoder} and \textbf{adaptive semantic transformation}. The representation generation module encodes the generated text into dense features and aggregates them effectively. The adaptive semantic transformation converts dense vectors from the semantic space to the recommendation space. It tackles the dimensionality mismatching and allows for noise mitigation. Thus, the knowledge adaptation stage increase the reliability and availability of the generated knowledge and bridging the gap between LLM and RS.
\subsubsection{Knowledge Encoder} To harness the potential of textual knowledge generated by LLMs, we employ a text encoder, usually another language model like BERT, to re-encode knowledge and get the encodings for each token within the text. Then, we require an aggregation process that combines the information from each tokens to generate preference representations $r^p_i\in\mathbb{R}^{m}$ and item knowledge representations $r^k_i\in\mathbb{R}^{m}$ of size $m$ as follows
\begin{equation}
    \begin{split}       
    &r^p_i = \text{Aggr}(\text{Encoder}(knowl^p_i))\,, \\
    &r^k_i = \text{Aggr}(\text{Encoder}(knowl^k_i))\,,
    \end{split}
\end{equation}
where $knowl^p_i$ and $knowl^k_i$ denote the textual preference knowledge and item knowledge generated by LLM of the $i$-th instance in dataset. Here, various aggregation functions can be employed, such as CLS token, last token, average pooling, and more. In the experimental section, we will explore and discuss the effectiveness of different aggregation methods. It is also important to note that if we have access to the dense vector outputs from LLM, the separate text encoder can be eliminated.
\subsubsection{Adaptive Semantic Transformation} In order to effectively utilize the aggregated representations obtained from the text encoder, we need to address three challenges: the high dimensionality of the representations, their placement in the semantic space rather than the recommendation space, and the noise issue. To tackle these issues, we introduce the Adaptive Semantic Transformation module. The aggregated representations capture diverse knowledge from multiple facets, so we employ a structure that mixing shared and dedicated experts, inspired by the Mixture of Experts (MoE)~\cite{MoE} approach. This allows us to fuse knowledge from different facets and benefits from the inherent robustness offered by the multiple experts. 

In particular, to fully exploit the shared information of the preference representation and the item knowledge representation, we have designed both shared experts and specific experts for each kind of representations. The shared experts capture the common aspects, such as shared features, patterns, or concepts, that are relevant to both preference and item knowledge. Each representation also has its dedicated set of experts to capture the unique characteristics specific to the preference or item knowledge. Mathematically, assuming that $SE$ and $DE$ are the sets of shared experts and dedicated experts with the expert number of $n_s$ and $n_d$, the transformed preference representation $\hat{r}_{i}^p\in\mathbb{R}^{q}$ and item knowledge representation $\hat{r}_{i}^k\in\mathbb{R}^{q}$ of size $q$ ($q$ is much less than the original dimension $m$) are calculated as follows
\begin{equation}
\begin{split}
    \alpha_{i}^p &=\operatorname{Softmax}(g^p(r^p_i))\,,\quad\alpha_{i}^k =\operatorname{Softmax}(g^k(r^k_i))\,,\\
    \hat{r}_{i}^p&=\sum\nolimits_{e\in SE} \alpha_{i,e} \times e(r^p_i) + \sum\nolimits_{e\in DE} \alpha_{i,e} \times e(r^p_i)\,,\\
    \hat{r}_{i}^k&=\sum\nolimits_{e\in SE} \alpha_{i,e} \times e(r^k_i) + \sum\nolimits_{e\in DE} \alpha_{i,e} \times e(r^k_i)\,,\\
\end{split}
\end{equation}
where $g^p(\cdot)$ and $g^k(\cdot)$ are the gating network for preference and item knowledge, and their outputs $\alpha^p_i$ and $\alpha^k_i$ are of the same size, $n_s+n_d$. Here $e(\cdot)$ denotes the expert network and $\alpha_{i,e}$ is the weight of expert $e(\cdot)$ generated by the gating network. Here, the experts are designed with Multi-Layer Perceptron (MLP), which facilitates dimensionality reduction and space transformation.

% PLE: share and specific experts
% \subsection{Prediction and Optimization}
\subsection{Knowledge Utilization}
Once we have obtained the transformed preference  representation and item knowledge representations, we can leverage them in traditional recommendation systems. In this section, we explore a preliminary approach where these representations are treated as additional input features. Taking the task of CTR prediction as an example, we incorporate both representations into the feature interaction layer, allowing them to interact effectively with other categorical features. During training and optimization, the adaptive semantic transformation module is jointly trained with the recommendation model to ensure that the transformation process adapts to the current data distribution. Importantly, the framework allows for different backbone CTR models and the original loss function of the CTR model remains unchanged, preserving its effectiveness in capturing click-through behavior. Therefore, the open-world knowledge-enhanced CTR framework can be formulated as 
\begin{equation}
    \hat{y_i} = f(x_i,h_i,\hat{r}_{i}^p,\hat{r}_{i}^k;\theta)\,.
     \label{eq:ctr-goal-3}
\end{equation}

This framework is also highly generalizable beyond CTR prediction, it can be extended to various recommendation tasks. By incorporating the transformed knowledge representations into the input layer, the framework allows for the utilization of both world knowledge and domain knowledge of RS in a unified manner. This enables the recommendation model to use the open-world knowledge provided by LLM easily and make more informed and personalized recommendations.
% backbone model, including but not limited to CTR model

\subsection{Speed-up Approach}
The above framework adopts LLMs to generate user preference knowledge and item knowledge. However, LLMs have a large number of parameters, often in the order of billions, and their inference take extensive computation time and resources. This results in the slower inference times of LLMs, which cannot meet the real-time requirements of recommendation scenarios. 

To address this, we employ a acceleration strategy to pre-store the knowledge repsentation $r^p_i$ and $r^k_i$ generated by LLM or text encoder in a database. During the inference stage of the backbone recommendation model, relevant representations are retrieved from the database. Since the characteristics of items often do not change frequently, obtaining item knowledge in advance is relatively straightforward. On the other hand, user behaviors evolve over time, making it challenging for LLM to provide real-time preference knowledge about behavioral changes. However, considering that long-term user preferences are stable, and the backbone model can typically leverage recent user history, we do not require LLM to have access to the most recent history. Instead, it can infer a user's long-term interests from slightly older historical data, while backbone model  focuses on capturing the user's short-term interests. 

Overall, pre-storing LLM-generated knowledge representations allows for efficient retrieval during recommendation inference, enabling the recommendation model to access relevant knowledge without relying on real-time LLM computations. The inclusion of pre-stored knowledge representations does not significantly increase the overall computational complexity of backbone model. Thus, the time complexity of the inference stage can be maintained at a level comparable to that of the original backbone model. Besides, this approach also strikes a balance between modeling long-term and short-term user interests, facilitating more accurate and timely recommendations.
% store and retrieval, cutting
% \subsubsection{Time Complexity} 
% almost the same

